On Evaluating Neural Network Backdoor Defenses

Deep neural networks (DNNs) demonstrate superior performance in various fields, including scrutiny and security. However, recent studies have shown that DNNs are vulnerable to backdoor attacks. Several defenses were proposed in the past to defend DNNs against such backdoor attacks. In this work, we conduct a critical analysis and identify common pitfalls in these existing defenses, prepare a comprehensive database of backdoor attacks, conduct a side-by-side evaluation of existing defenses against this database. Finally, we layout some general guidelines to help researchers develop more robust defenses in the future and avoid common mistakes from the past.

==> Workshop-NeurIPS 2020/a_intro.tex <==
\section{Introduction}\label{sec:intro}
\vspace{-0.75em}
%Deep neural networks (DNNs) are increasingly being
%used in many natural language processing~\cite{speech} and image recognition~\cite{image} tasks. 
%deployed in real-world safety-critical systems~\cite{8806018},  and as such,  are exposed to threats from the attackers. Recent work  has shown that DNNs are susceptible to test time adversarial perturbations and to training data poisoning or \textit{backdooring} attacks. 
%The robustness of DNNs against such attacks is a key concern. 
%While there is a relatively mature body of work on robustness to adversarial perturbations, backdooring defenses have only recently received attention. In this paper, we examine the growing body of literature on DNN backdooring defenses with a critical lens.
%especially on the more pernicious and recent attacks called backdoor attacks. Here, the attacker compromises both the test inputs and the DNN.

%DNNs can be compromised during training because users lack computational resources and/or high-quality training data; users often source the models to third party training~\cite{web} or download existing models from online model repositories~\cite{caffemodelzoo, modelzoo}. This creates an opening for an attacker to interfere with the training procedure and generate a malicious DNN (called ``BadNet''~\cite{badnets}) with a hidden backdoor. The attacker activates the backdoor using a trigger; a malicious modification of a test input that causes the DNN to misbehave in an attacker-chosen manner.
%in other words, classify the poisoned image (image with a trigger) as an attacker chosen target class while classifying clean inputs correctly. 

\begin{wraptable}{l}{0.55\textwidth}
\small
\vspace{-0.75em}
\begin{tabular}{lccc}
\toprule
Defense & Pitfall 1 & Pitfall 2 & Pitfall 3 \\
\midrule
Fine-pruning & \cmark & \xmark & \cmark \\
Neural Cleanse & \cmark & \cmark & \xmark \\
ABS & \xmark & \cmark & \cmark \\
STRIP & \xmark & \cmark & \xmark \\
Generative Modelling & \xmark & \cmark & \xmark \\
\bottomrule
\end{tabular}
\vspace{-0.25em}
\caption{Common pitfalls in existing defenses. Pitfall 1 is sensitivity to hyper-parameters, pitfall 2 is restrictive assumptions on backdoor structure and impact, and pitfall 3 is poor performance on adaptive attacks.}
\label{tab:pitfalls}
\vspace{-0.75em}
\end{wraptable}

Deep neural network backdooring attacks based on training data poisoning are an emerging and critical threat.
Several methods have been proposed recently to detect~\cite{tran2018spectral, strip2019acsac, absliu} and/or mitigate~\cite{neuralcleanse, finepruning, duke} backdoors. 
But, mirroring the early work on adversarial defenses, most backdooring defenses have been circumvented soon after publication. 
While this is often par for the course in security research, a critical analysis of existing defenses reveals common pitfalls that must be avoided in the search for a general and robust defense against backdooring attacks. Specifically, we found one or more of three common pitfalls in each defense we evaluated (see ~\autoref{tab:pitfalls}):
\begin{itemize}
    \item \textbf{Pitfall 1}: \textbf{Insufficient (or non-existent) evaluation against a range of attack hyper-parameters.} Empirically, we find that several defenses are highly sensitive choice of attack hyper-parameters, for instance, the learning rate used to train the BadNet. Several defenses fail to explore a range of hyper-parameters in their evaluation.
    \item \textbf{Pitfall 2}: \textbf{Restrictive assumptions on backdoor structure and impact.} Several defenses we evaluate assume that backdoor triggers are small, have fixed (and even known) size/shape, are additive in the pixel space, or only modify a region part of the input. Almost all defenses assume targeted "all-to-one" attacks, that is, backdoored images from any source class are mis-predicted as a single target class. In practice, however, attackers are far from being restricted to specific types of backdoors and can have a range of attack objectives. 
    
    % \akv{
    % Prior work limit their broad efficacy in mitigating backdoor behaviour by making restrictive assumptions. Here we list key limitations of prior work.
    % \begin{itemize}
    %     \item \textit{Assumptions on trigger properties:} Several defenses we evaluate assume that backdoor triggers are small, have fixed (and even known) size/shape, are additive in the pixel space, or only modify a region part of the input.
    %     \item \textit{Assumptions on target labels:} Almost all defenses assume targeted "all-to-one" attacks, that is, backdoored images from any source class are mis-predicted as a single target class.
    % \end{itemize}
    % }
    
    \item \textbf{Pitfall 3}: \textbf{Adaptive attacks that circumvent explicit defense assumptions not explored.} Finally, several defenses rely on explicit assumptions about how backdoors manifest in a network, but fail to examine if these assumptions can be easily circumvented. 
\end{itemize}
The pitfalls in existing work call into question the robustness of state-of-art defenses against backdooring attacks, and serve as a call-to-arms for more developing more general defenses that make minimal assumptions about the adversary. 

In this paper, we identify, qualitatively and empirically,  shortcomings in all existing state-of-art backdooring defenses related to one or more of the three pitfalls described above (\autoref{sec:pitfalls}), prepare a comprehensive database of BadNets attacks that encompass a range of attack hyper-parameters, backdoor types and attack objectives (\autoref{sec:setup}), and provide the first side-by-side evaluation of state-of-art defenses using the BadNet database (\autoref{sec:results}). We conclude by discussing marching orders for future defenses (\autoref{sec:discuss}). 
%These results are intended to spur research into generalizable defenses against backdooring attacks 

%\begin{itemize}
%    \item We identify, qualitatively and empirically,  shortcoming in all existing state-of-art backdooring defenses related to one or more of the three pitfalls described above (\autoref{sec:pitfalls}).
  %  \item We identify new attacks against existing defenses, and prepare a comprehensive database of BadNets attacks that encompass a range of attack hyper-parameters, backdoor types and attack objectives (\autoref{sec:setup}). The BadNet database will open-sourced to aid future evaluations of backdoor defenses.
    %\item We provide the first side-by-side evaluation of state-of-art defenses using the BadNet database (\autoref{sec:results}). We find that all defenses fail on atleast on attack in the database.
%\end{itemize}

% But almost all these works make unrealistic assumptions about the trigger nature and/or mechanics. Specifically the assumptions are that the trigger is small, location is fixed, shape and size are known a-priori and it does not cover the important features of the image. It is unclear how such an attack can be physically realized - for example, in face recognition system, the sunglasses trigger can be in a part of the image that the defender has no control over the size, shape and location. Focus is on semantically meaningful perturbations: typically in attacker controlled foreground, where the trigger is not necessarily small and can move around. Another line of work~\cite{absliu, finepruning} seeks to restrict neuronal activations in such a way that there exists neuron(s) that either activate only in the presence of a backdoor or the backdoored neurons work independently. Unfortunately, many existing defenses which encode these priors are shown to be effective only on simple attacks, where the attacker is constrained, and can be easily evaded by an advanced attacker. 

% In this paper, we discuss the necessity of developing strong defenses that make minimal assumptions and generalize to a wide range of backdoor attacks. Our specific contributions in this paper include:
% \paragraph{Contributions}
% \begin{itemize}
%     \item We review the existing state-of-the-art defenses in the literature.
%     \item We demonstrate the drawbacks of the existing defenses and exploit their weaknesses to design advanced BadNets.
%     \item We implement several advanced attacks: all-all attack, clean label attacks, attacks with variable location triggers, multi trigger - single target attack, multi trigger - multi target attack, feature space attacks and trigger combination attack. 
% \end{itemize}



==> Workshop-NeurIPS 2020/b_background.tex <==
\section{Threat Model}
\label{subsec:threatmodel}
\vspace{-0.75em}
Consistent with prior work, our threat model assumes an attacker with access to a large clean training data, $\mathcal{D}_{train}^{cl}$. Training benignly on this dataset produces a clean DNN, $f_{\theta_{cl}}$, with parameters ${\theta_{cl}}$ . However, the attacker's goal is to train a BadNet, $f_{\theta_{bd}}$, $\theta_{bd} \neq \theta_{cl}$, by poisoning the training data using function $\texttt{poison:} x^{cl} \rightarrow x^{p}$ and/or modifying the ground truth label of $x^{cl}$. Specifically, $f_{\theta_{bd}}$ is obtained by training on poisoned training data, $\mathcal{D}_{train}^{bd}$. The BadNet is trained such that $f_{\theta_{bd}}(x^{cl}) = f_{\theta_{cl}}(x^{cl})$, but $f_{\theta_{bd}}(x^{p})$ is not necessarily equal to  $f_{\theta_{cl}}(x^{cl})$. The attacker uploads $\theta_{bd}$ to an online model repositories where the user downloads the model and deploys it in the field after evaluating it on a small, held-out clean validation dataset, $\mathcal{D}_{valid}^{cl}$. (Tran et al.~\cite{tran2018spectral} assume a weaker model in which that the defender also has access to poisoned images in their threat model.) Importantly, the attacker has broad flexibility in choosing the $\texttt{poison}(\cdot)$ function from a range of physically plausible manipulations, and in determining how a BadNet misbehaves on poisoned inputs. We argue that a defense is incomplete unless it contends with the broadest possible class of attacks.
%for instance, it could m only on certain types of poisoned input, could map each poisoned source label to a different target label and so on.
%and target label, the defender has no access to it. So, the attacker can use a variety of attack strategies and in this paper, we consider several advanced attacks discussed in~\autoref{sec:setup}.

%The attacker's success is quantified in terms of the clean classification accuracy (CA), the BadNet's accuracy on clean inputs, and attack success rate (ASR), the BadNet's ability to achieve the attack objective on poisoned inputs. 

==> Workshop-NeurIPS 2020/c_pitfalls.tex <==
\section{Identifying Pitfalls in Existing Defenses}
\label{sec:pitfalls} 
\vspace{-0.75em}
Here we discuss the three pitfalls in prior work by giving prominent examples of each:

\vspace{-0.5em}
\subsection{Pitfall 1: Insufficient  (or  non-existent)  evaluation  against  a  range  of attack  hyper-parameters.}
\vspace{-0.75em}
\begin{wrapfigure}{R}{0.5\textwidth}
\centering
\subfloat{\label{fig:motiv-ada-neuron}\includegraphics[width=0.25\textwidth]{fig/fine-pruning/ada-neuron-crop.pdf}}
\subfloat{\label{fig:motiv-ada-prune}\includegraphics[width=0.25\textwidth]{fig/fine-pruning/ada-prune-crop.pdf}}
\caption {Shortcomings of fine pruning: Left plot is average neuron activations for each neuron in the last pooling layer, for a set of poisoned and benign inputs. Right plot shows the effect of pruning on clean accuracy and attack success.}
\vspace{-1.0em}
\label{fig:fine-pruning-fail}
\end{wrapfigure}

The \textit{Fine-pruning}~\cite{finepruning} defense is based on the observation that backdoor and clean inputs excite different neurons in a BadNet. However, this observation was based on BadNets trained with single set of hyper-parameters; by exploring a range of hyper-parameters including learning rate, batch size, weights initialization, data pre-processing, choice of optimizer, etc., we are able to find BadNets for which this assumption is violated. Consider~\autoref{fig:fine-pruning-fail}---while Fine-pruning is shown to be effective on BadNet (on sunglasses trigger) proposed in~\cite{finepruning}, it fails on the same BadNet trained with different hyper-parameters because backdoor neurons are also activated by clean inputs. 

%assumes that all neurons that are dormant on clean validation data are potentially backdoor neurons and prunes them. The BadNet weights are then fine-tuned using the validation dataset. In fact, BadNets can be trained such that backdoor and clean inputs have similar activation patterns, reducing efficacy of fine-pruning. Consider~\autoref{fig:fine-pruning-fail}---this illustrates Fine-pruning of two BadNets (on sunglasses trigger), one trained with the settings reported in~\cite{finepruning} and the other with different training hyper-parameters. Fine-pruning succeeds in the first case (see \autoref{fig:fine-pruning-fail} (a) and (b)) but fails in the second (see \autoref{fig:fine-pruning-fail} (c) and (d)) because backdoor neurons are also activated by clean inputs. Pruning therefore results in a large drop in clean accuracy, in this instance, even before the attack success rate starts declining. Further fine-tuning the pruned model with clean validation dataset will not reduce the attack success rate because clean data alone is not sufficient to activate all the backdoored neurons~\cite{veldanda2020nnoculation}.

% \begin{figure*}
% \centering
% \subfloat[Original BadNet]{\label{fig:motiv-adam-neuron}\includegraphics[width=0.25\textwidth]{fig/fine-pruning/adam-neuron-crop.pdf}}
% \subfloat[Original BadNet]{\label{fig:motiv-adam-prune}\includegraphics[width=0.25\textwidth]{fig/fine-pruning/adam-prune-crop.pdf}}\hfill
% \subfloat[Variant BadNet]{\label{fig:motiv-ada-neuron}\includegraphics[width=0.25\textwidth]{fig/fine-pruning/ada-neuron-crop.pdf}}
% \subfloat[Variant BadNet]{\label{fig:motiv-ada-prune}\includegraphics[width=0.25\textwidth]{fig/fine-pruning/ada-prune-crop.pdf}}
% \caption{Shortcomings of fine pruning: (a) and (c) plot the average neuron activations for each neuron in the last pooling layer, for a set of poisoned and benign inputs. (b) and (d) show the effect of pruning on clean accuracy and attack success.\label{fig:fine-pruning-fail}}
% \end{figure*}

\vspace{-0.5em}
\subsection{Pitfall 2: Restrictive assumptions on backdoor size, shape and impact.}
\vspace{-0.75em}
The NeuralCleanse defense makes restrictive assumptions on the backdoor size/shape while STRIP assumes that any backdoored input is always classified as a single target label. We discuss how these assumptions are easily subverted.

    \begin{wrapfigure}{R}{0.4\textwidth}
    \centering
    %\vspace{-2em}
    \includegraphics[width=0.4\textwidth]{fig/neural-fail-crop.png}
    \vspace{-1.5em}
    \caption {Shortcomings of NeuralCleanse applied to large trigger: Leftmost image is actual trigger; other images are incorrectly reverse-engineered triggers by NeuralCleanse.}
    \vspace{-1.0em}
    \label{fig:neural-fail}
    \vspace{-0.25em}
    \end{wrapfigure}
    
    \textbf{Assumptions on Trigger Shape and Size.} NeuralCleanse~\cite{neuralcleanse} and Qiao \textit{et al.}~\cite{duke} seeks to recover the trigger (or trigger distribution) given a BadNet; the recovered trigger (or distribution) is used (with corrected labels) to re-train the BadNet with the goal of disabling the backdoor~\cite{neuralcleanse,duke}. This is called \emph{backdoor unlearning}. To do so, however, NeuralCleanse~\cite{neuralcleanse} and Qiao \textit{et al.}~\cite{duke} assumes that the trigger is \emph{small} and \emph{contiguous} pattern super-imposed on a source image; e.g., the trigger could be a small fixed pattern of pixels superimposed in one corner of the image. 
 %   Qiao \textit{et al.}~\cite{duke} assume that the defender knows the trigger size and shape. These assumptions are unrealistic as:
    %\begin{itemize}
     %   \item the attacker chooses the trigger and has a \emph{vast} range of options for its shape and size, and
%        \item real-world triggers need not be small or contiguous as long as they are contextually meaningful --- e.g., in face recognition, sunglasses and lipstick of certain shades could together act as triggers~\cite{sunglassesattack}. Further, triggers need not super-positional either, for instance, feature space triggers~\cite{absliu} apply a filter on the entire image. %\findcite{cmu}
    %\end{itemize}
    
    %Consequently, prior works fail when the assumptions are not satisfied. 
    In practice, triggers need not be small or contiguous. For example, in~\autoref{fig:neural-fail} we illustrate the output from Neural Cleanse given BadNets triggered by a large, but semantically meaningful, sunglasses trigger for a face recognition application. The recovered triggers bear little resemblance to the original, missing its size, shape, and color

    \textbf{Assumptions on Backdoor Impact.}
    Except for fine-pruning, all the existing defenses work only for all-to-one attacks, i.e., they assume that backdoored inputs are mis-classified as a single target label, and cannot be easily generalized to a broader range of attacker objectives. For example, STRIP~\cite{strip2019acsac} assumes that any backdoored input is misclassified as the same target label and therefore, presence of a backdoor over-rides any other features of an input. Based on this assumption, STRIP  detects if test inputs are backdoored by passing a super-position of the test inputs with inputs from the validation set; the argument is that backdoored inputs will nevertheless get classified as the attacker-chosen target class, while clean inputs will be randomly mis-classified. However, in practice, a backdoor's impact can be input dependent;  for example, the target mis-classification depends on the class of the input as is the case for all-all attacks. We show in~\autoref{sec:results}, make it hard for STRIP to distinguish clean and backdoored inputs.
    
\vspace{-0.5em}
\subsection{Pitfall 3: Adaptive attacks that circumvent explicit defense assumptions not explored.}
\vspace{-0.75em}
A recent defense,  Artificial Brain Stimulation (ABS)~\cite{absliu} assumes that there exists a \emph{single} backdoor neuron in a BadNet that, when activated, independently causes all validation inputs to be classified as the target label and iteratively scans the network for such neurons. Networks in which such a backdoor neuron exists are marked as BadNets and are rejected. These assumptions do not always hold; in fact, BadNets can be trained such that multiple neurons must be activated to trigger the backdoor. For instance, consider a backdoor that is only triggered in the presence of a \emph{conjunction} of input features.  We demonstrate in ~\autoref{sec:results} that such a BadNet easily circumvents ABS. 


==> Workshop-NeurIPS 2020/d_exp_setup.tex <==
\section{Experimental Setup}\label{sec:setup}
\vspace{-0.75em}
We created BadNets encompassing a range of backdoor size/shapes and attack objectives as shown in ~\autoref{tab:exp_setup}. We also performed a hyper-parameter search to determine the most effective attacks.

\begin{table}
\tiny
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
BadNet & Attack Setting & Dataset & Trigger & Target label \\
\midrule
AAA~\cite{badnets} & All-All & \multirow{2}{*}{MNIST} & Patterned trigger & \multicolumn{1}{c}{\textit{y} $\rightarrow$ \textit{y+1}} \\   %why do we need the {2}*???? -- Mentioning 2 rows and center
CLA~\cite{cla_kang} & Clean-label &  & Fixed noise & 0 \\
\midrule
TCA & Trigger comb. & CIFAR-10 & Yellow triangle $+$ red square & 7 \\
\midrule
PN & Simple & \multirow{2}{*}{GTSRB} & Post-it note & 0 \\
FSA~\cite{absliu} & Feature Space &  & Gotham filter & 35 \\
\midrule
SG & Simple & \multirow{4}{*}{YouTube Face} & sg & 0 \\
LS & Simple &  & ls & 0 \\
MTSTA* & Multi-trigger, single target &  & ls, eb, sg & 4,4,4 \\
MTMTA* & Multi-trigger, multi target &  & ls, eb, sg & 1,5,8 \\
\midrule
\end{tabular}
}
\scriptsize{ \begin{flushleft} * for MTSTA and MTMTA, ls, eb, sg corresponds to lipstick, eyebrow, sunglasses trigger, respectively \end{flushleft}}
\caption{Details of BadNet attacks used to evaluate SOTA defenses.}
\label{tab:exp_setup}
\vspace{-2.5em}
\end{table}

A detailed description of the attacks is not possible due to space constraints, but we note that the TCA attack (that we propose) triggers only when \emph{both} a yellow triangle and red square are inserted in an image, while the MTSTA and MTMTA attacks trigger when the face image has \emph{either} lipstick, sunglasses or colored eyebrow. 


==> Workshop-NeurIPS 2020/e_results.tex <==
\section{Experimental Results}
\label{sec:results}
\vspace{-0.75em}

\begin{table*}[t]
\centering
\caption{Performance of existing defenses on baseline BadNets.
\label{tab:comparision_results}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccccc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{2}{c}{BadNet (Baseline)} & \multicolumn{2}{c}{Fine-Pruning} & \multicolumn{2}{c}{Neural Cleanse} & STRIP (FRR=3\%) & \multicolumn{2}{c}{Qiao \textit{et al.}~\cite{duke}} \\
BadNet & CA & ASR & CA & ASR & CA & ASR & FAR & CA & ASR \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10}
AAA & 97.76 & 95.91 & 97.6 & 57.35 & \multicolumn{2}{c}{Fails} & 99.22 & \multicolumn{2}{c}{Fails} \\
CLA & 89.02 & 100 & 99.13 & 14.68 & 97.74$^\dag$ & 4.77$^\dag$ & 43.45 & \multicolumn{2}{c}{-} \\
\midrule
TCA & 87.71 & 99.9 & 88.26 & 99.62 & 88.59$^\dag$ & 99.82$^\dag$ & 22.22 & \multicolumn{2}{c}{out of scope} \\
\midrule
PN & 95.46 & 99.82 & 94.58 & 99.69 & 95.24 & 12.39 & 100 & \multicolumn{2}{c}{out of scope} \\
FSA & 95.08 & 90.06 & 95.37 & 45.5 & 95.8 & 28.99 & 99.95 & 93.65$^\dag$ & 5.58$^\dag$ \\
\midrule
SG & 97.89 & 99.98 & 97.18 & 95.97 & 95.74$^\dag$ & 38.09$^\dag$ & 10.34 & 77.64$^\dag$ & 1.88$^\dag$ \\
LS & 97.19 & 91.51 & 97.86 & 90.53 & 97.14$^\dag$ & 28.44$^\dag$ & 18.42 & \multicolumn{2}{c}{out of scope} \\
MTSTA* & 95.84 & 92.22,92.24,100 & 97.31 & 45.04,64.71,94.94 & 93.37$^\dag$ & 0,0,8.67$^\dag$ & 11.79,63.73,5.84 & \multicolumn{2}{c}{out of scope} \\
MTMTA* & 95.93 & 91.51,91.39,100 & 96.91 & 52.36,82.34,0 & 94.18$^\dag$ & 30.79,0,95.68$^\dag$ & 15.90,53.64,15.58 & \multicolumn{2}{c}{out of scope} \\
\bottomrule
\end{tabular}
}
\scriptsize{ \begin{flushleft} * for MTSTA and MTMTA, the ASR corresponds to using lipstick, eyebrow, sunglasses trigger, respectively \end{flushleft}}
\scriptsize{ \begin{flushleft} $^\dag$ we give oracular knowledge to these defenses \end{flushleft}}
\vspace{-2.5em}
\end{table*}

We tabulate the results of our evaluation of five SOTA defenses in~\autoref{tab:comparision_results}. ABS data is not shown since we could only evaluate it for the TCA attack (ABS is available as an executable that works only on CIFAR-10 dataset and for a specific network architecture) for which it fails. None of the remaining defenses work across the board. Even if we generously set an ASR target of below $20\%$  for defense success, Fine-pruning only succeeds for CLA. Neural Cleanse succeeds for CLA, PN and MTSTA, but in two of the three cases, only if we give Neural Cleanse oracular knowledge of the target label. The success of Neural Cleanse on PN is to be expected since a Post-It Note trigger with a single target label fits squarely with its assumptions. STRIP only succeeds on the SG and LS BadNets, and as predicted, fails entirely on the AAA attack. Finally, the generative distribution modeling~\cite{duke} defense assumes that the trigger has a fixed size, shape and location, and that the size and location are known to the defender. Thus, attack settings with multiple triggers (MTMTA, MTSTA), non-contiguous triggers (TCA), and variable location triggers (PN, LS) are out-of-scope (i.e., there was no way for us to provide appropriate inputs about trigger size and location to the defense implementation). For the remaining attacks, the defense timed out (AAA) or failed to identify the correct target label.
    


%we could not evaluate ABS on other attack settings. Note that were unable to evaluate ABS on our attacks 
%The high-level take-home from our evaluation is that none of

   % \textbf{Fine-pruning}~\cite{finepruning} uses validation data to prune backdoor neurons and to retrain the pruned network. However, our BadNets contain neurons that are activated by both clean and backdoored inputs, thus causing Fine-pruning to fail in all but one instance to reduce ASR below $40\%$. Fine-pruning is most successful on the BadNet-CLA but still has $14\%$ ASR.
    
    %\textbf{Neural Cleanse}~\cite{neuralcleanse} by itself failed to detect the target label or reverse engineer the trigger on most of our BadNets. In these instances, we gave Neural Cleanse oracular knowledge of the target label, thus skewing the advantage in Neural Cleanse's favor. 
    %Nonetheless, we observe Neural Cleanse has poor performance on all but the PN, LS and MTSTA BadNets, although only when Neural Cleanse is given oracular knowledge for the latter two. The success of Neural Cleanse on BadNet-PN is to be expected since a Post-It Note trigger with a single target label fits squarely with its assumptions.
    
    %\textbf{STRIP}~\cite{strip2019acsac} is an online defense based on the observation that perturbing clean test inputs by superimposing randomly selected validation inputs will cause random mis-classification while doing the same with backdoored inputs causes the BadNet to typically output the attacker-chosen target label. 
    %However, this assumes a single target label; not surprisingly, STRIP does not work at all on BadNet-AAA (i.e., the all-to-all) since every label is a potential target. Further, STRIP also implicitly assumes that the trigger is strong enough to override the effect of other features in perturbed images---indeed, we find that STRIP is only reasonably effective on the single target BadNet-SG that uses large sunglasses as a trigger with an ASR of $10.34\%$.
    
    %\textbf{Generative Distribution Modeling}~\cite{duke} trains a generator to reverse engineer the trigger distribution for each target label and picks the target label most likely to correspond to a backdoor (i.e., it assumes a single target). 
    %This method assumes that the trigger has a fixed size, shape and location, and that the size and location are known to the defender. Thus, attack settings with multiple triggers (MTMTA, MTSTA), non-contiguous triggers (TCA), and variable location triggers (PN, LS) are out-of-scope (i.e., there was no way for us to provide appropriate inputs about trigger size and location to the defense implementation). For the remaining attacks, the defense timed out (AAA) or failed to identify the correct target label. Re-running the defense with oracular knowledge of the target label (we could not do this for AAA because it does not have a single target label) shows that the defense has low ASR for the FSA and SG attacks.
    
%    \begin{wrapfigure}{l}{0.45\textwidth}
  %  \centering
    %\vspace{-1.5em}
  %  \includegraphics[width=0.45\textwidth]{fig/abs/reversed_triggers.png}
    %\vspace{-1.5em}
    %\caption {ABS results of BadNet-TCA: The reverse engineered trigger in the (a) left image resembles a dog (label 5), (b) middle image resembles a horse (label 7) and (c) right image resembles the antlers of a deer (label 4)}
    %\vspace{-2.0em}
   % \label{fig:abs}
    %\end{wrapfigure}
    
   % \textbf{ABS}~\cite{absliu} critically relies on the assumption that a \emph{single} neuron controls the backdoor behavior. This assumption is easily circumvented by BadNet-TCA that uses a combination trigger that activates the backdoor only when \emph{both} triggers are present, i.e., more than one neuron is involved in encoding the backdoor behavior. 
    %Indeed, ABS fails on BadNet TCA: it outputs seven different reverse engineered triggers, none of which resemble the correct trigger; three of the reverse engineered triggers are shown in~\autoref{fig:abs}. 
    %We note that ABS marks an entire DNN as either backdoored or clean; in this case, ABS marks BadNet-TCA as clean. Since the ABS executable only works on the CIFAR-10 dataset and for a specific network architecture, we could not evaluate ABS on other attack settings. 
    %However, we note that like Neural Cleanse, ABS also critically relies on the assumption of a single target label that is activated if any input is backdoored---as such, we do not expect ABS to work well against multi-target attacks (AAA and MTMTA). 


==> Workshop-NeurIPS 2020/f_conclusion.tex <==
\section{Discussion and Conclusion}
\label{sec:discuss}
\vspace{-0.75em}

In this paper, we review the existing state-of-the-art defense techniques against backdoor attacks in DNNs. We identified three common pitfalls in prior defenses and show that as a consequence of these deficiencies none of the existing defenses currently work against a range of attacks. To address these shortcomings, we argue that future backdoor defenses should clearly address the following concerns:
%propose the following marching orders for future defenses:

\begin{itemize}
\item Explore a broad range of attack hyper-parameters: empirically, we found that BadNet properties can vary significantly depending on the hyper-parameters used to train the BadNets. Defenses that work for one set of hyper-parameters may not work for another. At the same time defenses have their own hyper-parameters. To characterize the inter-play between attackers and defender, defenses should seek to optimize both the attacker hyper-parameters to circumvent the defenses and, of course, vice-versa, using, for instance, the game theoretic equilibria between the attack and defense hyper-parameters. 
\item Propose defenses against a well-defined but broad range of threats: as we have shown, attacker's have an asymmetric advantage in selecting from a range of backdoors and backdoor impact. While it might be tempting to design defenses against specific backdoor types, for instance, small additive triggers that always cause an input to be mis-classified as a single target label, this often results in defenses that largely exploit properties of the specific attack and are hard to generalize to different attacks. It is hard to envision that the backdoor threat will be mitigated using piecemeal solutions for each different type of attack, and consequently we argue that defenses must seek to address the broadest possible range of attacks. 
\item Explore adaptive attacks: while an adaptive attack against a proposed defense is not always easy to design, authors should make a reasonable attempt to anticipate attacks against their proposed defenses, especially if the defense explicitly makes strong assumptions (for instance, that a single neuron encodes  a backdoor) and defenses do not easily generalize beyond that assumption.  
\end{itemize}

To conclude, we believe, based on our results, that there is plenty of important work left to be done in designing general and robust defenses against backdoor attacks. We hope that the future defenses will heed some of the warning signs that we highlight in this paper. From a practical standpoint, we plan to make all attacks developed as part of this paper publicly available to aid in the evaluation of future defenses. 

